Hallucinated Adversarial Control for Conservative Offline Policy Evaluation

We study the problem of conservative off-policy evaluation (COPE) where given an offline dataset of environment interactions, collected by other agents, we seek to obtain a (tight) lower bound on a policy's performance. This is crucial when deciding whether a given policy satisfies certain minimal performance/safety criteria before it can be deployed in the real world. To this end, we introduce HAMBO, which builds on an uncertainty-aware learned model of the transition dynamics. To form a conservative estimate of the policy's performance, HAMBO hallucinates worst-case trajectories that the policy may take, within the margin of the models' epistemic confidence regions. We prove that the resulting COPE estimates are valid lower bounds, and, under regularity conditions, show their convergence to the true expected return. Finally, we discuss scalable variants of our approach based on Bayesian Neural Networks and empirically demonstrate that they yield reliable and tight lower bounds in various continuous control environments.

==> dump_old_writing.tex <==
\subsection{OLD WRITING}

HAMBO is a model-based method.
Therefore, we first train a transition model $p_\theta$ on the data $\calD_b$.
We use an ensemble of Gaussian neural networks that capture the mean and aleatoric uncertainty of the transition dynamics. Specifically, 
we train $K\in\mathbb{N}$ networks that predict the mean and variance of the target.
Therefore we get for all $s,a \in \mathcal{S} \times \mathcal{A}$ a set $\{(\mu_{\theta_k}(s,a), \Sigma_{\theta_k}(s,a))\}_{k=1}^K$ where for all $k \in [K]$ the vector $\mu_{\theta_k}(s,a)$ and the matrix $\Sigma_{\theta_k}(s,a)$ represent mean and covariance respectively.
For practical and scalability reasons we consider diagonal covariance matrices.

The $K$ networks are trained together via Stein variational gradient descent \cite{liu2016svgd} to obtain a good representation of the posterior $p(\theta|\calD_b)$. 
We capture the epistemic uncertainty via the discrepancy between the individual ensemble members. 

\begin{algorithm}
\label{algorithm:hambo}
\caption{HAMBO}
\begin{algorithmic}[1]
\REQUIRE offline dataset $\calD_b$, policy $\pi$
\ENSURE (conservative) estimate of expected return $J(\pi)$
\STATE split $\calD_b$ into $D_t$, $D_e$, $D_c$
\WHILE{recent improvement on $D_e$}
\STATE train $p_\theta$ one epoch on $D_t$ via SVGD
\ENDWHILE
\STATE recalibrate $p_\theta$ on $D_c$ using temperature scaling
\STATE train adversary $\eta$ for induced model environment
\STATE rollout $\pi$ using $p_\theta$ and $\eta$ to get estimates
\end{algorithmic}
\end{algorithm}

Once the transition model $p_\theta$ is learned, the policy $\pi$ is evaluated/rolled out on the model. Accordingly, in every timestep, a sample from $p_\theta$ is taken.
Here \textsc{HAMBO} uses the epistemic uncertainty of the model to obtain a sample for the next state which is conservative with respect to the expected returns. 


There are multiple methods for how the $K$ Gaussian distributions of our model can be used for sampling \cite{chua2018pets} and a unique way to introduce conservatism for every method.
The following paragraphs describe the neutral and conservative variants of said methods.

\paragraph{Trajectory Sampling Infinity (TSInf)}
A simple sampling method is to choose an index $k \in \{1,...,K\}$ at the beginning of an episode and only use that model of the ensemble.
More precisely for the entire episode, we have
\begin{align*}
y_{t+1} \sim \mathcal{N}(\mu_{\theta_k}(s_t,a_t), \Sigma_{\theta_k}(s_t,a_t))
\end{align*}
for all $t \in [T-1]$.
To get a good estimate of the return this is done for all the ensemble members and the results are averaged.

In order to get conservative estimates this is also done for all $k \in \{1,...,K\}$ but the worst result is picked (or the appropriate quantile) instead of taking the average.

\paragraph{Trajectory Sampling 1 (TS1)}
The prediction of the ensemble can be thought of as a mixture of Gaussians.
It is natural to choose uniform weights.
In that case, every timestep sampling would be done by first choosing an index from $[K]$ uniformly at random and then sampling according to that model of the ensemble.
That is
\begin{align*}
k &\sim \mathcal{U}(\{1,...,K\})\\
y_{t+1} &\sim \mathcal{N}(\mu_{\theta_k}(s_t,a_t), \Sigma_{\theta_k}(s_t,a_t))
\end{align*}
for all $t\in [T-1]$.

To achieve conservatism in TS1 the index can be chosen adversarially instead of randomly.
So sampling for the next state is done via
\begin{align*}
k &\sim \eta(s_t,a_t)\\
y_{t+1} &\sim \mathcal{N}(\mu_{\theta_k}(s_t,a_t), \Sigma_{\theta_k}(s_t,a_t))
\end{align*}
for all $t\in [T-1]$, where the adversary $\eta$ is trained to minimise the return.
This can be done using a normal reinforcement learning algorithm on the induced model environment with negative reward.
We use the clipped double DQN algorithm \cite{fujimoto2018td3}.

\paragraph{Distribution Sampling (DS)}
Instead of interpreting the mixture of Gaussians, the members of the ensemble can be aggregated via moment matching to get one Gaussian distribution.
Formally the sampling would then be done via
\begin{align*}
y_{t+1} \sim \mathcal{N}(\mu_\theta(s_t,a_t), \Sigma_\theta(s_t,a_t))
\end{align*}
where (with $(s_t,a_t)$ omitted for readability)
\begin{align*}
\mu_\theta &= \frac{1}{K}\sum_{k=1}^K\mu_{\theta_k}\\
\Sigma_\theta &= \underbrace{\frac{1}{K}\sum_{k=1}^K(\mu_{\theta_k}-\mu_\theta)(\mu_{\theta_k}-\mu_\theta)^T}_{:=\Sigma_\theta^e} + \underbrace{\frac{1}{K}\sum_{k=1}^K\Sigma_{\theta_k}}_{:=\Sigma_\theta^a}
\end{align*}
for all $t \in [T-1]$.
We can define the epistemic part of the variance $\Sigma_\theta^e$ as the first summand and the aleatoric one $\Sigma_\theta^a$ as the second summand.

Note that because the individual members of the ensemble are trained to fit the target distribution themselves and not after aggregation the DS variant has the tendency to be underconfident and predict too large variance.
To counteract this the model is recalibrated on a dedicated calibration set $D_c \subset \calD_b$ using temperature scaling \cite{kuleshov2018calibration}.

Conservatism for the DS variant can be achieved as in H-UCRL \cite{curi2020hucrl} and RH-UCRL \cite{curi2021rhucrl}.
That is to have again an adversary $\eta$ that is allowed to modify the mean prediction within some confidence interval according to the epistemic uncertainty.
Formally the sampling for the next state is done via
\begin{align*}
y_{t+1} \sim \mathcal{N}(\mu_\theta(s_t,a_t) + \beta^{\sfrac{1}{2}} S_\theta^e(s_t,a_t)\eta(s_t,a_t), \Sigma_\theta^a(s_t,a_t))
\end{align*}
for all $t\in [T-1]$, where $\mu_\theta$ and $\Sigma_\theta^a$ are defined as above and $S_\theta^e(s,a) = \diag(\sigma_\theta^e(s,a))$ with $\sigma_\theta^e(s,a)$ being the vector containing the square roots of the diagonal elements of $\Sigma_\theta^e(s,a)$ as introduced above.

The hallucinated policy $\eta$ can again be trained on the induced model environment with negative reward.
We use the SAC algorithm \cite{haarnoja2018sac,haarnoja2018sac2} for that.

\section{Theoretical Analysis}
\label{section:theory}

In this section theoretical properties of \textsc{HAMBO} are established for the DS variant.
The reasoning is inspired by the work on H-UCRL \cite{curi2020hucrl}.
For missing proofs, we defer to Appendix \ref{sec:missingproofs}.

For the derivation of meaningful properties, some assumptions have to be made.

\begin{assumption}
\label{assumption:mdp}
We have an MDP $\mathcal{M} = (\mathcal{S}, \mathcal{A}, p, p_0, T)$ with $\mathcal{S} \subseteq \mathbb{R}^{d_s}$ and $\mathcal{A} \subseteq \mathbb{R}^{d_a}$ for some $d_s,d_a \in \mathbb{N}$ and where $p$ is such that the reward is deterministic $r_{t+1} = r(s_t,a_t)$ and the next state can be determined as $s_{t+1} = f(s_t,a_t) + \epsilon_t$ for all $t \in [T-1]$ where the $\epsilon_t$ are aleatoric noise such that $\epsilon_{0:T-1} =: \epsilon \sim p_a$ for some distribution $p_a$ from which we can sample.
\end{assumption}

\begin{assumption}[Calibrated model]
\label{assumption:calibrated}
The learned transition model $p_\theta$ is well calibrated.
That is with probability $(1-\delta)$ for some $\delta \in (0,1)$ it holds jointly for all $s,a \in \mathcal{S}\times\mathcal{A}$ that elementwise $|f(s,a)-\mu_\theta(s,a)| \leq \beta^{\sfrac{1}{2}}\sigma_\theta^e(s,a)$.
Here $f$ is defined as in Assumption~\ref{assumption:mdp}.
\end{assumption}

While in general, neural network based models are not calibrated, they can be recalibrated \cite{kuleshov2018calibration} to satisfy Assumption \ref{assumption:calibrated} as described in Section \ref{section:method}.






